Affinity and Diversity: Quantifying Mechanisms of Data Augmentation

Though data augmentation has become a standard component of deep neural network training, the underlying mechanism behind the effectiveness of these techniques remains poorly understood. In practice, augmentation policies are often chosen using heuristics of either distribution shift or augmentation diversity. Inspired by these, we seek to quantify how data augmentation improves model generalization. To this end, we introduce interpretable and easy-to-compute measures: Affinity and Diversity. We find that augmentation performance is predicted not by either of these alone but by jointly optimizing the two.

==> Augmentation Taxonomy for arxiv v2/abstract.tex <==
% "Abstracts must be a single paragraph, ideally between 4–6 sentences long."
\begin{abstract}
Though data augmentation has become a standard component of deep neural network training, the underlying mechanism behind the effectiveness of these techniques remains poorly understood. In practice, augmentation policies are often chosen using heuristics of either distribution shift or augmentation diversity. Inspired by these, we seek to quantify how data augmentation improves model generalization. To this end, we introduce interpretable and easy-to-compute measures: \indistness{} and \diversity{}. We find that augmentation performance is predicted not by either of these alone but by jointly optimizing the two. 
\end{abstract}

==> Augmentation Taxonomy for arxiv v2/acknowledgments.tex <==
% \begin{ack}
\section*{Acknowledgements}
The authors would like to thank  Alex Alemi, Justin Gilmer, Guy Gur-Ari, Albin Jones, Behnam Neyshabur, Zan Armstrong, and Ben Poole for thoughtful discussions on this work. 

% \end{ack}

==> Augmentation Taxonomy for arxiv v2/broaderimpact.tex <==
\section{Broader Impact}
\paragraph{Data augmentation has the potential to amplify bias}
\*

Data augmentation takes a smaller, potentially biased training set and recycles this as the basis of a larger augmented training program. A central finding of this work is that the success of an augmentation policy varies with the dual metrics of \indistness{} and \diversity{}; as \indistness{} is explicitly model-dependent, it depends on biases present in the model.
This data reuse and model-dependence of successful augmentation suggest the possibility that augmentation may amplify biases in the data or model and warrants future investigation. 

\paragraph{Robust data augmentation can reduce social, environmental, and financial costs}
\*

At its best, data augmentation provides a means for less well-funded or data-rich practitioners to design performant models by supplementing a smaller training data set with additional transformed images.
Commonly-used policies, however, such as those found by AutoAugment~\cite{cubuk2018autoaugment} have relied on expensive brute force searches which cost thousands of GPU-hours, replacing the need for extensive data collections with the need for financially and environmentally expensive compute.
We hope that by understanding the mechanisms behind successful data augmentation we can design guided augmentation policies for new datasets and models, and mitigate the social and financial costs of data collection without undue compute expense. 
\paragraph{Fundamental understanding facilitates impact assessment}
\*

More broadly, the central aim of this work is to better understand the elements driving successful augmentation policies. Truly understanding the conceptual mechanisms at play is crucial in making informed judgements about the impact of data augmentation.
 

% \paragraph{Fundamental understanding facilitates impact assesment}




% With our insights of how augmentations work, we can potentially lowering this computational cost by, for instance:
% 1) guiding an automatic policy search algorithm by setting \indistness{} and \diversity{} as a direct objective, potentially making the search much easier.
% 2) steering the creation of human-made single augmentations to increase \diversity{}, creating more effective single augmentations.

% The use of data augmentation in machine learning systems is widespread. As these systems start being deployed and affecting people in the real world, it is crucial that we have a better understanding of the impacts, intended or not, of these systems on the people they affect. This task is made much harder when we don't understand the systems themselves, and what possible unintended consequences of their uses are, which is the case for most deep learning systems. 

% Our work focuses on analysing and understanding the mechanism through which data augmentations work in an effort to introduce science to the widespread practice. In particular, we focus on single transformations in order to build a foundation for this data augmentation science. This way, we contribute to the collective body of knowledge on how these systems work, and could impact people.

% In addition to this, our work has more direct, practical impacts. Our findings have the potential to enable the easy creation of data augmentation policies. Commonly used policies such as those found by AutoAugment~\cite{cubuk2018autoaugment} relied on expensive parameter searches which cost thousands of GPU-hours. With our insights of how augmentations work, we can potentially lowering this computational cost by, for instance:
% 1) guiding an automatic policy search algorithm by setting \indistness{} and \diversity{} as a direct objective, potentially making the search much easier.
% 2) steering the creation of human-made single augmentations to increase \diversity{}, creating more effective single augmentations.

==> Augmentation Taxonomy for arxiv v2/conclusion.tex <==
\newpage
\section{Conclusion}
\vspace{-0.1in}%
We attempted to quantify common intuition that more in-distribution and more diverse augmentation policies perform well. To this end, we introduced two easy-to-compute metrics, \indistness\ and \diversity{}, intended to measure to what extent a given augmentation is in-distribution and how complex the augmentation is to learn. Because they are model-dependent, these metrics capture the data shifts that affect model performance.

With these tools, we have conducted a study over a large class of augmentations for \cifar\ and \imagenet\ and found that neither feature alone is a perfect predictor of performance.
Rather, we presented evidence that \diversity\ and \indistness\ play dual roles in determining augmentation quality. Optimizing for either metric separately is sub-optimal and the best augmentations balance the two.

Additionally, we found that an increased number of training examples, connected to \diversity{}, was a necessary ingredient of beneficial augmentation.

Finally, we found that augmentations share an important feature with other regularizers: switching off regularization at the right time can improve performance. In some cases, this can cause an otherwise poorly-performing augmentation to be beneficial.

We hope our findings provide a foundation for continued scientific study of data augmentation. 

==> Augmentation Taxonomy for arxiv v2/discussion.tex <==
\section{Discussion}%
\vspace{-0.15in}%
In this work, we focused on single transforms in an attempt to understand the essential parts of augmentation in a controlled context. This builds a foundation for using these metrics to quantify and design more complex and powerful combinations of augmentations. 

Though earlier work has often explicitly focused on just one of these metrics, chosen priors have implicitly ensured reasonable values for both. One way to achieve \diversity{} is to use combinations of many single augmentations, as in AutoAugment \citep{cubuk2018autoaugment}. Because transforms and hyperparameters in~\citet{cubuk2018autoaugment} were chosen by optimizing performance on proxy tasks, the optimal policies include high and low \indistness{} transforms. 
Fast AutoAugment~\citep{lim2019fast}, CTAugment~\citep{berthelot2019remixmatch, sohn2020fixmatch}, and differentiable RandAugment~\citep{cubuk2019randaugment} all aim to increase \indistness{} by what \citet{lim2019fast} called ``density-matching''. However these methods use the search space of AutoAugment and thus inherit its \diversity{}. 

On the other hand, Adversarial AutoAugment~\cite{zhang2019adversarial} focused on increasing \diversity{} by optimizing policies to increase the training loss. While this method did not explicitly aim to increase \indistness{}, it also used transforms and hyperparameters from the AutoAugment search space. Without such a prior, which includes useful \indistness{}, the goal of maximizing training loss with no other constraints would lead to data augmentation policies that erase all the information from the images. 

Our results motivate casting an even wider net when searching for augmentation strategies. Firstly, our work suggests that explicitly optimizing along axes of both \indistness{} and \diversity{} yields better performance. Furthermore, we have seen that poor-performing augmentations can actually be helpful if turned off during training (Fig.~\ref{fig:slingshot}). With inclusion of scheduling in augmentation optimization, we expect there are opportunities for including a different set of augmentations in an ideal policy. \citet{ho2019population} observes trends in how probability and magnitude of various transforms change during training for an optimized augmentation schedule. We suggest that with further study, \diversity{} and \indistness{} can provide priors for optimization of augmentation schedules. 

==> Augmentation Taxonomy for arxiv v2/introduction.tex <==
\begin{figure}[ht]
% \vspace{-0.3in} % make 0.2 in case this format is too crowded
\vskip 0.1in 
\begin{center}
\centerline{%
    \hfill%
    \begin{subfigure}[\indistness{} vs \diversity{}]{%
        \includegraphics[width=0.41\columnwidth]{figures/header/header_cifar_pareto_new_invert_notrel_affinity_arxiv.pdf}%
    }\end{subfigure}%
    \hfill%
    \begin{subfigure}[Model's View of Data]{%
        \includegraphics[width=0.41\columnwidth]{figures/header/indist_diversity_venn_newdata_newsize_blue_labeled_nodash_grey_quad.pdf}%
    }\end{subfigure}%
    \hfill%
}%
\caption{\small {\bf \indistness{} and \diversity{} parameterize the performance of a model trained with augmentation}. (a) \cifar{}: Color shows the final test accuracy. * marks the clean baseline. Each point represents a different augmentation that yields test accuracy greater than 88.7\%. (b) Representation of how clean data and augmented data are related in the space of these two metrics. Higher diversity is represented by a larger bubble while distributional similarity is depicted through the overlap of bubbles.
Test accuracy generally improves to the upper right in this space. Adding real new data to the training set is expected to be in the far upper right corner.}
\label{fig:header}
\end{center}
\vskip -0.1in
% \vspace{-0.3in}
\end{figure}

% \begin{wrapfigure}[]{r}{0.58\columnwidth}%[ht]
% \vspace{-0.6in} % make 0.2 in case this format is too crowded
% \vskip 0.1in 
% \begin{center}
% \centerline{%
%     \begin{subfigure}[\indistness{} vs \diversity{}]{%
%         \includegraphics[width=0.29\columnwidth]{figures/header/header_cifar_pareto_new_invert_notrel_affinity_arxiv.pdf}%
%     }\end{subfigure}%
%     \hfill%
%     \begin{subfigure}[Model's View of Data]{%
%         \includegraphics[width=0.29\columnwidth]{figures/header/indist_diversity_venn_newdata_newsize_blue_labeled_nodash_grey_quad.pdf}%
%     }\end{subfigure}%
% }%
% \caption{\small {\bf \indistness{} and \diversity{} parameterize the performance of a model trained with augmentation}. (a) \cifar{}: Color shows the final test accuracy. * marks the clean baseline. Each point represents a different augmentation that yields test accuracy greater than 88.7\%. (b) Schematic representation of how clean data and augmented data are related to each other in the space of these two metrics. Higher data diversity is represented by a larger bubble while distributional similarity is depicted through the overlap between bubbles.
% Test accuracy generally improves to the upper right in this space. Adding real new data to the training set is expected to be in the far upper right corner.}
% \label{fig:header}
% \end{center}
% \vskip -0.1in
% \vspace{-0.2in}
% \end{wrapfigure}

\section{Introduction}
\vspace{-0.1in}%
Models that achieve state-of-the-art in image classification often use heavy data augmentation strategies.
The best techniques use various transforms applied sequentially and stochastically. Though the effectiveness of this is well-established, the mechanism through which these transformations work is not well-understood. 

Since early uses of data augmentation, it has been assumed that augmentation works because it simulates realistic samples from the true data distribution: ``[augmentation strategies are] reasonable since the transformed reference data is now extremely close to the original data. In this way, the amount of training data is effectively increased"~\citep{Bellegarda1992}. Because of this, augmentations have often been designed with the heuristic of incurring minimal distribution shift from the training data.

This rationale does not explain why unrealistic distortions such as cutout~\citep{cutout2017}, SpecAugment~\citep{park2019specaugment}, and mixup~\citep{zhang2017mixup} significantly improve generalization performance. 
Furthermore, methods do not always transfer across datasets---\aug{Cutout}, for example, is useful on \cifar{} and not on \imagenet{}~\citep{lopes2019improving}. 
Additionally, many augmentation policies heavily modify images by stochastically applying multiple transforms to a single image.
Based on this observation, some have proposed that augmentation strategies are effective because they increase the diversity of images seen by the model.

In this complex landscape, claims about diversity and distributional similarity remain unverified heuristics. Without more precise data augmentation science, finding state-of-the-art strategies requires brute force that can cost thousands of GPU hours~\citep{cubuk2018autoaugment, zhang2019adversarial}. This highlights a need to specify and measure the relationship between the original training data and the augmented dataset, as relevant to a given model's performance.

In this paper, we quantify these heuristics. Seeking to understand the mechanisms of augmentation, we focus on single transforms as a foundation. We present an extensive study of 204 different augmentations on \cifar\ and 223 on \imagenet{}, varying both broad transform families and finer transform parameters. Our contributions are:
\begin{enumerate}%
\item We introduce \indistness{} and \diversity{}: interpretable, easy-to-compute metrics for parameterizing augmentation performance. \indistness\ quantifies how much an augmentation shifts the training data distribution from that learned by a model.
\diversity{} quantifies the complexity of the augmented data with respect to the model and learning procedure. 
\item We show that performance is dependent on {\it both} metrics. In the \indistness{}-\diversity{} plane, the best augmentation strategies jointly optimize the two (see Fig~\ref{fig:header}).
\item We connect augmentation to other familiar forms of regularization, such as $\ell_{2}$ and learning rate scheduling, observing common features of the dynamics: performance can be improved and training accelerated by turning off regularization at an appropriate time. 
\item We show that performance is only improved when a transform increases the total number of unique training examples. 
The utility of these new training examples is informed by the augmentation’s \indistness{} and \diversity{}.
\end{enumerate}%


==> Augmentation Taxonomy for arxiv v2/methods.tex <==
\section{Methods}\label{Sec:methods}
\vspace{-0.1in}%
We performed extensive experiments with various augmentations on \cifar{} and \imagenet{}.
Experiments on \cifar{} used the WRN-28-2 model \cite{WRN2016}, trained for 78k steps with cosine learning rate decay. Results are the mean over 10 initializations and reported errors (often too small to show on figures) are the standard error on the mean. Details on the error analysis are in Sec.~\ref{sec:error}.

Experiments on \imagenet{} used the ResNet-50 model~\cite{he2016deep}, trained for 112.6k steps with a weight decay rate of 1e-4, and a learning rate of 0.2, which is decayed by 10 at epochs 30, 60, and 80.

Images were pre-processed by dividing each pixel value by 255 and normalizing by the data set statistics. Random crop was also applied on all \imagenet{} models.
These pre-processed data without further augmentation are ``clean data'' and a model trained on it is the ``clean baseline''. We followed the same implementation details as~\citet{cubuk2018autoaugment}\footnote{Available at \texttt{bit.ly/2v2FojN}}, including for most augmentation operations. Further implementation details are in Sec.~\ref{sec:training}.

For \cifar{}, test accuracy on the clean baseline is $89.7\pm0.1\%$. The validation accuracy is $89.9\pm0.2\%$. On \imagenet{}, the test accuracy is 76.06\%.

Unless specified otherwise, data augmentation was applied following standard practice: each time an image is drawn, the given augmentation is applied with a given probability. We call this mode \emph{dynamic} augmentation. Due to whatever stochasticity is in the transform itself (such as randomly selecting the location for a crop) or in the policy (such as applying a flip only with 50\% probability), the augmented image could be different each time. Thus, most of the tested augmentations increase the number of possible distinct images that can be shown during training.

We also performed select experiments using \emph{static} training. In static augmentation, the augmentation policy (one or more transforms) is applied once to the entire clean training set. Static augmentation does not change the number of unique images in the dataset.

\subsection{\indistness: a simple metric for distribution shift}
\vspace{-0.1in}%
Thus far, heuristics of distribution shift have motivated design of augmentation policies. Inspired by this focus, we introduce a simple metric to quantify how augmentation shifts data {\it with respect to the decision boundary of the clean baseline model}.

We start by noting that a trained model is often sensitive to the distribution of the training data. That is, model performance varies greatly between new samples from the true data distribution and samples from a shifted distribution. 

Importantly, the model’s sensitivity to distribution shift is not purely a function of the input data distribution, since training dynamics and the model’s implicit biases affect performance. Because the goal of augmentation is improving model performance, measuring shifts with respect to the distribution captured by the model is more meaningful than measuring shifts in the distribution of the input data alone. 

We thus define \indistness\ to be the difference between the validation accuracy of a model trained on clean data and tested on clean data, and the accuracy of the same model tested on an augmented validation set. Here, the augmentation is applied to the validation dataset in one pass, as a static augmentation. More formally we define:
\begin{definition}%
Let ${D}_{\textrm{train}}$ and ${D}_{\textrm{val}}$ be training and validation datasets drawn IID from the same \emph{clean} data distribution, and let ${D}'_{\textrm{val}}$ be derived from ${D}_{\textrm{val}}$ by applying a stochastic augmentation strategy, $a$, once to each image in ${D}_{\textrm{val}}$, ${D}'_{\textrm{val}}=\{(a(x), y)\ :\forall\ (x,y)\in{D}_{\textrm{val}}\}$. Further let $m$ be a model trained on ${D}_{\textrm{train}}$ and $\mathcal{A}(m,{D})$ denote the model's accuracy when evaluated on dataset ${D}$. The \indistness, $\mathcal{T}[a;m;{D}_\textrm{val}]$, is given by
\begin{align}
    \mathcal{T}[a; m; {D}_\textrm{val}]=\mathcal{A}(m,{D}'_\textrm{val}) - \mathcal{A}(m,{D}_\textrm{val})\,.
\end{align}
\end{definition}%
With this definition, \indistness\ of zero represents no shift and a negative number suggests that the augmented data is out-of-distribution for the model.

\begin{figure}[ht]
\vspace{-0.2in}
\vskip 0.1in % their example skipped 0.2in but only skip of 0.1in required
\begin{center}
\begin{minipage}[l]{0.5\textwidth}
    % \centerline{%
        \begin{subfigure}[\indistness]{%
            \includegraphics[width=0.5\columnwidth]{figures/toy_example/typicality_ref_small_edge}%
        }\end{subfigure}%
        \hfill%
        \begin{subfigure}[$D_{\textrm{KL}}$]{%
            \includegraphics[width=0.5\columnwidth]{figures/toy_example/KL_ref_small_edge}%
        }\end{subfigure}%
    % }%
    % \vspace{-0.1in}
\end{minipage}\hfill
\raisebox{0.2in}{
\begin{minipage}[c]{0.48\textwidth}
    \caption{\small {\bf \indistness{} is a model-sensitive measure of distribution shift}. Contours indicate lines of equal (a) \indistness{}, or (b) KL Divergence between the joint distribution of the original data and targets and the shifted data. The two axes indicate the actual shifts that define the augmentation. \indistness{} captures model-dependent features, such as the decision boundary.}
    \label{fig:toy_metrics}
\end{minipage}
}
\end{center}
% \vskip -0.1in
\vspace{-0.2in}
\end{figure}

In Fig.~\ref{fig:toy_metrics} we illustrate \indistness{} with a two-class classification task on a mixture of two Gaussians. Augmentation in this example comprises shift of the means of the Gaussians of the validation data compared to those used for training. Under this shift, we calculate both \indistness{} and KL divergence of the shifted data with respect to the original data. \indistness{} changes only when the shift in the data is with respect to the model's decision boundary, whereas the KL divergence changes even when data is shifted in the direction that is irrelevant to the classification task. In this way, \indistness{} captures what is relevant to a model: shifts that impact predictions.

This same metric has been used as a measure of a model's robustness to image corruptions that do not change images' semantic content \citep{azulay2018deep, dodge2017study,ford2019adversarial,hendrycks2018benchmarking,  rosenfeld2018elephant, yin2019afourier}. Here we, turn this around and use it to quantify the shift of augmented data compared to clean data.

\indistness{} has the following advantages as a metric:%
\begin{enumerate}%
%\vspace{-0.09in}%
\item It is easy to measure. It requires only clean training of the model in question. %
%\vspace{-0.05in}
\item It is independent of any confounding interaction between the data augmentation and the training process, since augmentation is only used on the validation set and applied statically.%
%\vspace{-0.05in}
\item It is a measure of distance sensitive to properties of both the data distribution \emph{and} the model.%
% \vspace{-0.09in}%
\end{enumerate}%

We gain confidence in this metric by comparing it to other potential model-dependant measures of distribution shift. We consider the mean log likelihood of augmented test images\citep{grathwohl2019energyclassifier}, and the Watanabe–Akaike information criterion (WAIC) \citep{WAIC}. These other metrics have high correlation with \indistness{}. Details can be found in Sec.~\ref{sec:supplsewaic}.

% -----------------------------------------------------------------------------
\subsection{Diversity: A measure of augmentation complexity}
\vspace{-0.1in}%
Inspired by the observation that multi-factor augmentation policies such as \aug{FlipLR}+\aug{Crop}+\aug{Cutout} and \aug{RandAugment}\citep{cubuk2019randaugment} greatly improve performance, we propose another axis on which to view augmentation policies, which we dub \emph{\diversity}. This measure is intended to quantify the intuition that augmentations prevent models from over-fitting by increasing the number of samples in the training set; the importance of this is shown in Sec.~\ref{sec:fixedaug}.

Based on the intuition that more diverse data should be more difficult for a model to fit, we propose a model-based measure. The \diversity{} metric in this paper is the final training loss of a model trained with a given augmentation:
\begin{definition}\label{defn:diversity}
Let $a$ be an augmentation  and $D_{\textrm{train}}'$ be the augmented training data resulting from applying the augmentation, $a$, stochastically. Further, let $L_{\textrm{train}}$ be the training loss for a model, $m$, trained on $D_{\textrm{train}}'$. We define the \diversity, $\mathcal{D}[a;m;D_{\textrm{train}}]$, as
\begin{align}
    \mathcal{D}[a;m;D_{\textrm{train}}]&:=\mathbb{E}_{ D_{\textrm{train}}'}\left[L_{\textrm{train}}\right]\,.
\end{align}
\end{definition}

Though determining the training loss requires the same amount of work as determining final test accuracy, here we focus on this metric as a tool for understanding. 

As with \indistness{}, this definition of \diversity{} has the advantage that it can capture model-dependent elements, i.e. it is informed by the class of priors implicit in choosing a model and optimization scheme as well as by the stopping criterion used in training.

Another potential diversity measure is the entropy of the transformed data, $\mathcal{D}_{\textrm{Ent}}$. This is inspired by the intuition that augmentations with more degrees of freedom perform better. For discrete transformations, we consider the conditional entropy of the augmented data.
\begin{align}
    \mathcal{D}_{\textrm{Ent}}\,:=\,H(X'|X)\,=\,-\mathbb{E}_{X}\left[\Sigma_ {x'} p(x'|X)\log(p(x'|X))\right]\,.\nonumber
\end{align}
Here $x\in X$ is a clean training image and $x' \in X'$ is an augmented image. This measure has the property that it can be evaluated without any training or reference to model architecture. However, the appropriate entropy for continuously-varying transforms is less straightforward. 

A third proxy for \diversity{} is the training time needed for a model to reach a given training accuracy threshold. In Sec.~\ref{sec:divmetrics}, we show that these three metrics correlate well with each other.

In the remaining sections we describe how the complementary metrics of \diversity\ and \indistness\ can be used to characterize and understand augmentation performance.

%---------------------------


==> Augmentation Taxonomy for arxiv v2/related.tex <==
\section{Related Work}\label{Sec:related}
\vspace{-0.1in}%
Since early uses of data augmentation in training neural networks, there has been an assumption that effective transforms for data augmentation are those that produce images from an ``overlapping but different" distribution~\cite{bengio2011deep, Bellegarda1992}.
Indeed, elastic distortions as well as distortions in the scale, position, and orientation of training images have been used on \mnist~\cite{ciregan2012multi,sato2015apac,simard2003best,wan2013regularization}, while horizontal flips, random crops, and random distortions to color channels have been used on \cifar{} and \imagenet{}~\cite{krizhevsky2012imagenet,WRN2016, zoph2017learning}.
For object detection and image segmentation, one can also use object-centric cropping~\cite{liu2016ssd} or cut-and-paste new objects~\cite{dwibedi2017cut, fang2019instaboost, ngiam2019starnet}.

In contrast, researchers have also successfully used more generic transformations that are less domain-specific, such as Gaussian noise~\cite{ford2019adversarial, lopes2019improving}, input dropout~\cite{srivastava2014dropout}, erasing random patches of the training samples during training~\cite{cutout2017, park2019specaugment, zhong2017random}, and adversarial noise~\cite{szegedy2013intriguing}. Mixup~\cite{zhang2017mixup} and Sample Pairing~\cite{inoue2018data} are two augmentation methods that use convex combinations of training samples. 

It is also possible to improve generalization by combining individual transformations. For example, reinforcement learning has been used to choose more optimal combinations of data augmentation transformations~\cite{ratner2017learning, cubuk2018autoaugment}. Follow-up research has lowered the computation cost of such optimization, by using population based training~\cite{ho2019population}, density matching~\cite{lim2019fast}, adversarial policy-design that evolves throughout training~\cite{zhang2019adversarial}, or a reduced search space~\cite{cubuk2019randaugment}. Despite producing unrealistic outputs, such combinations of augmentations can be highly effective in different tasks~\cite{berthelot2019remixmatch,tan2019efficientnet, tan2019efficientdet, xie2019adversarial, xie2019unsupervised}.

Across these different examples, the role of distribution shift in training remains unclear.
\citet{lim2019fast,hataya2019faster} have found augmentation policies by minimizing the distance between the distributions of augmented data and clean data. Recent work found that after training with augmented data, fine-tuning on clean training data can be beneficial~\citep{He2019switching}, while \citet{touvron2019fixing} found it beneficial to fine-tune with a test-set resolution that aligns with the training-set resolution. 

The true input-space distribution from which a training dataset is drawn remains elusive. To better understand the effect of distribution shift on model performance, many works attempt to estimate it. Often these techniques require training secondary models, such as those based on variational methods ~\citep{NIPS2014_5423, kingma2014autoencoding, nowozin2016fgan, Blei_2017}. Others have tried to augment the training set by modelling the data distribution directly~\cite{tran2017bayesian}.
Recent work has suggested that even unrealistic distribution modelling can be beneficial~\citep{dai2017good}.

These methods try to specify the distribution separately
from the model they are trying to optimize. As a result, they are insensitive to any interaction between the model and data distribution. Instead, we are interested in a measure of how much the data shifts along directions that are most relevant to the model's performance.



==> Augmentation Taxonomy for arxiv v2/results.tex <==
\section{Results}
\vspace{-0.1in}%
\subsection{Augmentation performance is determined by both \indistness{} and \diversity{}}
\vspace{-0.1in}%
Despite the original inspiration to mimic realistic transformations and minimize distribution shift, many state-of-the-art augmentations yield unrealistic images.
This suggests that distribution shift alone does not fully describe or predict augmentation performance.

\begin{figure}[ht]
    \centering%
    \begin{subfigure}[T: \cifar{}. B: \imagenet{}]{%
        \begin{minipage}[b]{0.3\columnwidth}%
            % NOTE:  for the includegraphics below, 0.86in == 0.5\columnwidth (no longer true)
            \includegraphics[height=0.72in]{figures/distr_shift_correlation/indistness_cifar_noinset_tiny_purple_invert_affinity_arxiv.pdf}%
            \includegraphics[height=0.72in, clip, trim={0.5cm 0 0 0}]{figures/distr_shift_correlation/diversity_cifar_noinset_tiny_purple_invert_arxiv.pdf}%, 
            \vskip 0pt\vspace{-0.1in}%
            \includegraphics[height=0.72in]{figures/distr_shift_correlation/indistness_imagenet_noinset_tiny_new_purple_affinity.pdf}%
            \includegraphics[height=0.72in, clip, trim={0.5cm 0 0 0}]{figures/distr_shift_correlation/diversity_imagenet_noinset_tiny_new_purple.pdf}%
            \vspace{0.1in}
         \end{minipage}%
         \label{huge-a}
    }\end{subfigure}%
    \hfill%
    \begin{subfigure}[\cifar{}]{%
         \includegraphics[width=0.34\columnwidth]{figures/main_fig/cifar_div_ind_main_new_invert_notrel_affinity_arxiv.pdf}%
         \label{huge-b}
    }\end{subfigure}%
    \hfill%
    \begin{subfigure}[\imagenet{}]{%
         \includegraphics[width=0.34\columnwidth]{figures/main_fig/imagenet_div_ind_main_new_invert_notrel_affinity.pdf}%
         \label{huge-c}
    }\end{subfigure}%
    \caption{\small {\bf Augmentation performance is determined by both \indistness{} and \diversity{}}. (a) Test accuracy plotted against each of \indistness{} and \diversity{} for the two datasets, showing that neither metric alone predicts performance. In the \cifar{} plots (top), blue highlights (also in inset) are the augmentations that increase test accuracy above the clean baseline. Dashed lines indicate the clean baseline. (b) and (c) show test accuracy on the color scale in the plane of \indistness{} and \diversity{}. The three star markers in (b) are (left to right) \aug{RandAugment}, \aug{AutoAugment}, and \aug{mixup}. The * on the color bar indicates the clean baseline case. For fixed values of \indistness{}, test accuracy generally increases with higher values of \diversity{}. For fixed values of \diversity{}, test accuracy generally increases with higher values of \indistness{}. Note that the gains observed on \imagenet{} are expected to be small, in line with previous work on single-transformation policies~\cite{yin2019afourier}.}
    \label{fig:mainhugefig}
    % \vskip -0.02in
\end{figure}

Figure~\ref{huge-a} (left) measures \indistness\ across 204 different augmentations for \cifar\ and 223 for \imagenet\ respectively. We find that for the most important augmentations---those that help performance---\indistness\ is a poor predictor of accuracy. Furthermore, we find many successful augmentations with low \indistness{}. For example, \aug{Rotate(fixed, 45deg, 50\%)}, \aug{Cutout(16)}, and combinations of \aug{FlipLR}, \aug{Crop(32)}, and \aug{Cutout(16)} all have \indistness{}$<-15\%$ and test accuracy$>2\%$ above clean baseline on \cifar{}. Augmentation details are in Sec.~\ref{sec:augdetails}.

As \indistness{} does not fully characterize the performance of an augmentation, we seek another metric. To assess the importance of an augmentation's complexity, we measure \diversity\ across the same set of augmentations. We find that \diversity{} is complementary in explaining how augmentations can increase test performance. As shown in Fig.~\ref{huge-b} and \subref{huge-c}, \indistness\ and \diversity\ together provide a much clearer parameterization of an augmentation policy's benefit to performance. For a fixed level of \diversity, augmentations with higher \indistness\ are consistently better. Similarly, for a fixed \indistness, it is generally better to have higher \diversity{}.

A simple case study is presented in Fig.~\ref{fig:rotate_case_study}. The probability of the transform \aug{Rotate(fixed, 60deg)} is varied. The accuracy and \indistness\ are not monotonically related, with the peak accuracy falling at an intermediate value of \indistness. Similarly, accuracy is correlated with \diversity{} for low probability transformations, but does not track for higher probabilities. The optimal probability for \aug{Rotate(fixed, 60deg)} lies at an intermediate value of \indistness{} and \diversity{}.

\begin{figure}[ht]
\vskip 0.1in % their example skipped 0.2in but only skip of 0.1in required
\vspace{-0.2in}
\begin{center}
\centerline{%
    \raisebox{15 pt}{
        \begin{subfigure}{%
            % \begin{minipage}[b]{0.175\columnwidth}%
            \includegraphics[width=0.23\columnwidth]{figures/case_study/rotate_affinity_lines_new_arxiv.pdf}%
                % \vskip 0pt%
        }\end{subfigure}%
        \begin{subfigure}{%
            \includegraphics[width=0.23\columnwidth]{figures/case_study/rotate_diversity_lines.pdf}%
            %  \end{minipage}%
        }\end{subfigure}%
    }
    % \raisebox{20 pt}{
        \begin{subfigure}{%
            \includegraphics[width=0.35\columnwidth]{figures/case_study/rotate_affinity_diversity_lines_new_arxiv.pdf}% prev width: 0.375
        }\end{subfigure}%
    % }
}%
\vspace{-0.1in}%
\caption{\small {\bf Test accuracy varies differently than either \indistness{} or \diversity}. Here, the probability of \aug{Rotate(fixed, 60deg)} on \cifar{} is varied from 10\% to 90\%. Left: as probability increases, \indistness{} decreases linearly while the accuracy changes non-monotonically. Center: accuracy and \diversity\ vary differently from each other as probability is changed. Right: test accuracy is maximized at intermediate values.}
\label{fig:rotate_case_study}
\end{center}
\vskip -0.2in
\end{figure}

To situate the tested augmentations---mostly single transforms---within the context of the state-of-the-art, we tested three high-performance augmentations from literature: \aug{mixup} ~\citep{zhang2017mixup}, \aug{AutoAugment} \citep{cubuk2018autoaugment}, and \aug{RandAugment}~\citep{cubuk2019randaugment}. These are highlighted with a star marker in Fig.~\ref{huge-b}.

More than either of the metrics alone, \indistness{} and \diversity{} together provide a useful parameterization of an augmentation's performance. 
We now turn to investigating the utility of this tool for explaining other observed phenomena of data augmentations.

\subsection{Turning augmentations off may adjust \indistness{}, \diversity{}, and performance}
\vspace{-0.1in}%

The term ``regularizer'' is ill-defined in the literature, often referring to any technique used to reduce generalization error without necessarily reducing training error~\citep{Goodfellow-et-al-2016}. With this definition, it is widely acknowledged that commonly-used augmentations act as regularizers~\citep{hernandez2018further,zhang2016understanding,dao2019kernel}. 
Though this is a broad definition, we notice another commonality across seemingly different kinds of regularizers:
various regularization techniques yield boosts in performance (or at least no degradation) if the regularization is \textit{turned off} at the right time during training. For instance:%
%
\begin{enumerate}%
    %\vspace{-1.0 pt}%
    \item Decaying a large learning rate on an appropriate schedule can be better than maintaining a large learning rate throughout training~\citep{WRN2016}.%
    %\vspace{-0.05in}%
    \item Turning off $\ell_{2}$ regularization at the right time in training does not hurt performance~\citep{golatkar2019time}.%
    %\vspace{-0.05in}%
    \item Relaxing architectural constraints mid-training can boost final performance~\citep{dascoli2019CNNtoFCN}.%
    %\vspace{-0.05in}%
    \item Turning augmentations off and fine-tuning on clean data can improve final test accuracy~\citep{He2019switching}.%
    %\vspace{-1.0 pt}%
\end{enumerate}%
%
To further study augmentation as a regularizer, we compare the constant augmentation case (with the same augmentation throughout) to the case where the augmentation is turned off partway through training and training is completed with clean data. For each transform, we test over a range of switch-off points and select the one that yields the best final validation or test accuracy on \cifar{} and \imagenet{} respectively. The Switch-off Lift is the resulting increase in final test accuracy, compared to training with augmented data the entire time. 

\begin{figure}[ht!]
\vskip 0.1in 
\begin{center}
    \begin{subfigure}[Slingshot effect on \cifar{}]{
        \includegraphics[width=0.45\columnwidth]{figures/switch_aug_and_reg_off/switch_dynamics_notitle_ell_new_large.pdf}%
        \label{slingshot-a}
    }\end{subfigure}
    \begin{minipage}[b]{0.45\columnwidth}
        \begin{subfigure}[Switch-off Lift on \cifar{}]{
            \includegraphics[width=\columnwidth]{figures/switch_aug_and_reg_off/switching_slopegraph_blue_shaddow.pdf}%
            \label{slingshot-b}
        }\end{subfigure}
        \hfill %
        \begin{subfigure}[\cifar{} (left) \imagenet{} (right)]{
            \includegraphics[width=0.495\columnwidth]{figures/switch_aug_and_reg_off/cifar_switching_switch_nobox_arxiv.pdf}%
            \includegraphics[width=0.495\columnwidth]{figures/switch_aug_and_reg_off/imagenet_switching_switch_new.pdf}%
            \label{subfig:switching_DnI}
        }\end{subfigure}%
    \end{minipage}
% }
\caption{\small {\bf \subref{slingshot-a} Switching off regularizers yields a performance boost}: Three examples of how turning off a regularizer increases the validation accuracy. This slingshot effect can speed up training and improve the best validation accuracy. Top: training with no augmentation (clean baseline), compared to constant augmentation, and augmentation that is turned off at 55k steps. Here, the augmentation is \aug{Rotate(fixed, 20deg,100\%)}. Middle: Baseline with constant $\ell_{2}$. This is compared to turning off $\ell_{2}$ regularization part way through training. Bottom: Constant learning rate of 0.1 compared to training where the learning rate is decayed in one step by a factor of 10.
{\bf \subref{slingshot-b} Bad augmentations can become helpful if switched off}: Colored lines connect the test accuracy with augmentation applied throughout training (top) to the test accuracy with switching mid-training. Color indicates the amount of Switch-off Lift; blue is positive and orange is negative.
{\bf \subref{subfig:switching_DnI} Switch-off Lift varies with \indistness{} and \diversity{}}. Where Switch-off Lift is negative, it is mapped to 0 on the color scale.}
\label{fig:slingshot}
\end{center}
\vskip -0.1in
\vspace{-0.15in}
\end{figure}

For some poor-performing augmentations, this gain can actually bring the final test accuracy above the baseline, as shown in Fig.~\ref{slingshot-b}. We additionally observe (Fig.~\ref{slingshot-a}) that this test accuracy improvement can happen quite rapidly for both augmentations and for the other regularizers tested. This suggests an opportunity to accelerate training without hurting performance by appropriately switching off regularization. We call this a \emph{slingshot} effect.

Interestingly, we find the best time for turning off an augmentation is not always close to the end of training, contrary to what is shown in \citet{He2019switching}. For example, without switching, \aug{FlipUD(100\%)} decreases test accuracy by almost 50\% compared to clean baseline. When the augmentation is used for only the first third of training, final test accuracy is above the baseline.

\citet{He2019switching} hypothesized that the gain from turning augmentation off is due to recovery from a distribution shift. Indeed, for many detrimental transformations, the test accuracy gained by turning off the augmentation merely recovers the clean baseline performance. However, in Fig.~\ref{subfig:switching_DnI}, we see that for a given value of \indistness{}, Switch-off Lift can vary. This result suggests that the Switch-off Lift is derived from more than simply correction of a distribution shift.

% \begin{wrapfigure}{r}{0.4\columnwidth}%[ht]
% \vskip -0.1in 
% \vspace{-0.1in}
% \begin{center}
% \includegraphics[width=0.4\columnwidth]{figures/fixed_aug/static_comparison_purple_invert_big.pdf}
% \caption{\small {\bf Static augmentations never improve performance}. On \cifar{}, static augmentation performance on tested augmentations is less than the clean baseline, $(0,0)$, and less than the dynamic augmentation case. Diagonal line indicates where static augmentation would equal dynamic augmentation. Augmentations with no stochasticity are excluded because they are trivially equal on the two axes.}
% \label{fig:fixedaug}
% \end{center}
% \vskip -0.1in
% \vspace{-0.5in}
% \end{wrapfigure}


A few of the tested augmentations, such as \aug{FlipLR(100\%)}, are fully deterministic. Thus, each time an image is drawn in training, it is augmented the same way. When such an augmentation is turned off partway through training, the model then sees images---the clean ones---that are now new. Indeed, when \aug{FlipLR(100\%)} is switched off at the right time, its final test accuracy exceeds that of \aug{FlipLR(50\%)} without switching. In this way, switching augmentation off may adjust for not only low \indistness{} but also low \diversity{}. 

% ------------------------------------------------------------------------------------

\subsection{Increased effective training set size is crucial for data augmentation}\label{sec:fixedaug}
\vspace{-0.1in}%

Most augmentations we tested and those used in practice have inherent stochasticity and thus may alter a given training image differently each time the image is drawn. In the typical \emph{dynamic} training mode, these augmentations increase the number of unique inputs seen across training epochs.

To further study how augmentations act as regularizers, we seek to discriminate this increase in effective dataset size from other effects. We train models with \emph{static} augmentation, as described in Sec.~\ref{Sec:methods}. This altered training set is used without further modification during training so that the number of unique training inputs is the same between the augmented and the clean training settings.

For almost all tested augmentations, using static augmentation yields lower test accuracy than the clean baseline. Where static augmentation shows a gain (versions of \aug{crop}), the difference is less than the standard error on the mean. As in the dynamic case, poorer performance in the static case is for transforms that have lower \indistness{} and lower \diversity{}. 

Static augmentations also always perform worse than their non-deterministic, dynamic counterparts, as shown in Fig.~\ref{fig:fixedaug}. This may be because the \diversity{} of a static augmentation is always less than the dynamic case (see also Sec.~\ref{sec:divmetrics}). The decrease in \diversity{} in the static case suggests a connection between \diversity{} and the number of training examples. 
\begin{figure}[h]
\vspace{-0.1in}
\hspace{-0.1in}
\begin{minipage}[l]{0.6\textwidth}
    \hspace{-0.1in}\includegraphics[width=0.5\columnwidth]{figures/fixed_aug/static_comparison_purple_invert_big.pdf}%
    \includegraphics[width=0.5\columnwidth]{figures/supplement_figs/diversityerror.pdf}
\end{minipage}
\raisebox{0.15in}{
    \begin{minipage}[l]{0.4\textwidth}
        % \hspace{-0.2in}%
        \caption{\small {\bf Static augmentations decrease diversity and performance}. \cifar{}, static augmentation performance is less than the clean baseline, $(0,0)$, and less than the dynamic augmentation case. Augmentations with no stochasticity are excluded because they are trivially equal on the two axes (left). \diversity{} in the static case is less than in the dynamic case.(right) Diagonal line indicates where static and dynamic cases would be equal. }\label{fig:fixedaug}
    \end{minipage}}
\vspace{-0.1in}
\end{figure}

Together, these results point to the following conclusion: \textit{Increased effective training set size is crucial to the performance benefit of data augmentation. An augmentation's \indistness{} and \diversity{} inform how useful the additional training examples are.}
 
% ------------------------------------------------------------------------------------


